Minibatch and Momentum Model-based Methods for Stochastic Weakly Convex Optimization

Stochastic model-based methods have received increasing attention lately due to their appealing robustness to the stepsize selection and provable efficiency guarantee. We make two important extensions for improving model-based methods on stochastic weakly convex optimization. First, we propose new minibatch model-based methods by involving a set of samples to approximate the model function in each iteration. For the first time, we show that stochastic algorithms achieve linear speedup over the batch size even for non-smooth and non-convex (particularly, weakly convex) problems. To this end, we develop a novel sensitivity analysis of the proximal mapping involved in each algorithm iteration. Our analysis appears to be of independent interests in more general settings. Second, motivated by the success of momentum stochastic gradient descent, we propose a new stochastic extrapolated model-based method, greatly extending the classic Polyak momentum technique to a wider class of stochastic algorithms for weakly convex optimization. The rate of convergence to some natural stationarity condition is established over a fairly flexible range of extrapolation terms. While mainly focusing on weakly convex optimization, we also extend our work to convex optimization. We apply the minibatch and extrapolated model-based methods to stochastic convex optimization, for which we provide a new complexity bound and promising linear speedup in batch size. Moreover, an accelerated model-based method based on Nesterov's momentum is presented, for which we establish an optimal complexity bound for reaching optimality.

==> sec_cvx.tex <==
\section{Convex Optimization}
In this section, we further analyze the convergence of {\smod} methods for convex optimization.
\begin{enumerate}
	\item $f_x(\cdot,\xi)$ is a convex, 
	\item $f_y(x,\xi)\le f(x,\xi)$,
	\item $f(x,\xi)\le f_y(x,\xi) +\frac{\tau}{2}\|x-y\|^2$. 
\end{enumerate}


==> sec_introduction_long.tex <==
\section{Introduction}

In this paper, we are interested in the following optimization problem
\begin{mini}
{x\in\Xcal}{f(x)= \Expe_{\xi\sim\Xi} \big[f(x,\xi)\big]}{}{}\label{prob:main}
\end{mini}
where $f(\cdot,\xi)$ is sub-differentiable and possibly non-convex,
$\xi$ follows some unknown probability distribution $\Xi$, and $\Xcal$
is a convex closed set. Stochastic (sub)gradient descent~({\sgd}) is
the most widely used algorithm for solving the above problem, and
it has been successfully applied to many important applications such
as deep learning and many other supervised learning models \cite{RN312},
and widely deployed in mainstream numerical computing libraries, e.g.
\cite{abadi2016tensorflow}.


While tremendous work has been done to make {\sgd} more effective, far
less work is known for problems where the objective is both\textit{
non-smooth and non-convex}. Recently, an important progress was made
by\,\cite{duchi2018stochastic,davis2019stochasticweakly}, who proposed
stochastic model-based ({\smod}) methods for  weakly convex
optimization, a class of non-smooth non-convex problems with a wide range
of applications such as phase retrieval, robust PCA, low rank decomposition,
among others. Due to the flexibility of choosing the model functions,
{\smod} encompasses not only {\sgd}, but also many other popular proximal
algorithms including prox-linear (Gauss-Newton) and proximal point.
A precise characterization of model function will be given in Section~\ref{sec:background}.
Moreover, the work \cite{duchi2018stochastic,davis2019stochasticweakly}
show promising theoretical results: both asymptotic convergence and
rate of convergence to stationarity are established for the whole
family of stochastic model-based methods, despite the fact that the
problem lacks differentiability. Additionally, experiments
show that {\smod} often outperforms {\sgd} and exhibits a remarkable robustness to the hyper-parameters.

While the recent work suggests that {\smod}
is a competitive alternative to {\sgd}, our theoretical understanding
of this new scheme is far from complete. Particularly, we address the following potential limitations of the current approach in non-smooth and non-convex optimization.

\paragraph*{Minibatch}

Minibatch stochastic algorithms are widely deployed to leverage the
computing power of modern parallel architectures. For smooth optimization,
it is well known that batch size is a free parameter and it can linearly
reduce the iteration count of {\sgd}. See  \cite{dekel2012optimal,saeed-lan-nonconvex-2013,takavc2015distributed}.
However, for non-smooth optimization, our  understanding
of minibatches is rather limited. For non-convex composite optimization
where the nonsmooth part is simple,%
{} standard analysis of stochastic proximal gradient requires an exceedingly large batch size
(i.e. dependent on iteration count and target accuracy) to obtain
convergence efficiency guarantee. (cf. \cite{ghadimi2016mini}). To
alleviate this issue, \cite{davis2019stochasticweakly} developed
a novel complexity analysis of SGD and {\smod}, different from the classic
convergence analysis in the choice of Lyapunov (potential) function.
{} However, in the presence of non-smoothness, the complexity of {\smod}
is $\Ocal(L^{2}/\vep^{4})$, where $L$ is the Lipschitz constant
of the model function. Since this bound does not involve the batch
size, it is unclear how the complexity is influenced by
minibatching. This raises the question about whether minibatches can
help for stochastic non-smooth non-convex optimization. If the answer
is yes, can we provide an improved analysis of stochastic optimization
in the minibatch setting?

\paragraph*{Momentum}

Momentum techniques, such as the Polyak's heavy ball\,\cite{RN316}
and Nesterov's accelerated gradient\,\cite{RN185}, are widely used
in stochastic optimization of machine learning and deep learning models
\cite{RN312,he2016deep}.
Recently, the work~\cite{yan2018a} gave a unified convergence analysis of stochastic
gradient and stochastic momentum for unconstrained smooth non-convex
optimization. Subsequently, the study\,\cite{liu2020improved,defazio2020understanding}
further improved the convergence rate of stochastic momentum method
based on a novel Lyapunov analysis. In \cite{pmlr-v119-mai20b}, the
authors presented the first complexity analysis of stochastic heavy-ball
method for optimizing weakly convex problems. However, to the best
of our knowledge, despite considerable amount of work on momentum
{\sgd}, there is no momentum variant of other stochastic model-based
methods such as prox-linear and proximal point. Thus, it is natural
to ask the question: can we develop a momentum based model-based method,
with provable complexity guarantee, for stochastic non-smooth and non-convex
optimization?


\paragraph*{Contributions}

In this paper, we address the aforementioned questions and make novel extensions of stochastic model-based
methods as follows.

 We study the minibatch stochastic model-based methods and develop sharper rates of convergence to stationarity, providing a nearly-complete recipe on when minibatching would be helpful in the presence of nonsmoothness. 
For instance, (proximal) {\sgd} has linear speedup over minibatching as long as the loss is smooth, which includes the composite problems with nonsmooth regularizers such as $\ell_1$-penalty or constrained problems. 
Hence, our study answers the question about whether minibatch can linearly improve the iteration complexity of {\sgd} beyond unconstrained smooth optimization. 
Moreover, our theory shows that stochastic proximal point can be linearly accelerated by minibathcing, and stochastic proximal-linear has the same promising speedup for composition functions (illustrated in Section~\ref{sec:minibatch}).
To the best of our knowledge, this is the first analysis
 showing that these minibatch stochastic algorithms achieve linear speedup over the batch size even for \textit{non-smooth} and \textit{non-convex} optimization. 
 
 Our second contribution is a new technique to analyze the convergence of minibatch algorithms. We exploit an interesting connection between stochastic optimization and algorithm stability. 
While stability is traditionally used to show the generalization of learning algorithms, 
we real the magic power of stability theory in algorithm convergence from a pure optimization perspective. More specific, we show that  proximal mappings, involved in each iteration of stochastic algorithms, are stable in the sense that the outcome does not change too much when the minibatch is modified slightly.
By characterizing such perturbation error carefully, we develop a much sharper complexity bound  and clearly identify how batch size affects the convergence rates.
Notably, our new convergence analysis is substantially different from the standard variance-based analysis for minibatch SGD, which  only explains the effectiveness of minibatching in unconstrained smooth optimization. 


 We present new extrapolated model-based methods by incorporating a momentum term of Polyak type. 
We develop a unified Lyapunov analysis to show that a worst-case complexity of $\Ocal(1/\vep^{4})$ holds for all momentum {\smod} algorithms. 
To the best of our knowledge, these are the first complexity results of momentum based stochastic  prox-linear and proximal point algorithms for non-smooth non-convex optimization.
Our theory also guarantees a similar  complexity bound of  momentum {\sgd} and its proximal extension, thereby being more general than the recent work~\cite{pmlr-v119-mai20b}, which only proves convergence of momentum projected {\sgd}. 
We remark a potential advantage of our work over \cite{pmlr-v119-mai20b} via the application of composite optimization, for which the nonsmooth term is often involved via its proximity operator rather than its subgradient.
Consider in Lasso problem, to enhance solution sparsity, it is often favorable to invoke the proximity operator of $\ell_1$ function (Soft-thresholding). Our analysis can be easily applied for proximal {\sgd}  with momentum while the work \cite{pmlr-v119-mai20b} may not be appropriate due to its explicit requirement of the subgradient of the whole objective.


\textbf{Other related work}
There has been a continuous interest in stochastic non-smooth optimization
in the past few decades. While earlier work studied asymptotic convergence
\cite{ruszczynski1980feasible, ruszczynski1986method}, recent work
put more emphasis on the non-asymptotic complexity analysis \cite{davis2019stochasticweakly,pmlr-v119-mai20b}.
In the convex setting, minibatch stochastic model-based methods have
been studied in \cite{asi2020minibatch}. However, to guarantee speedup
in the non-smooth problems, they require a strong assumption
of restricted strong convexity, and their proof technique does not
extend readily to the non-convex setting. On the practical side, robustness
and fast convergence of model-based optimization were shown on many
non-smooth non-convex statistical learning problems \cite{charisopoulos2019low,duchi2019solving,asi2019the}.
Advantages of model based methods over stochastic gradient descent
for training deep neural networks were examined in \cite{charisopoulos2019low,berrada2019deep,frerix2018proximal,botev2017practical}.
Momentum techniques are widely used in modern practice of machine
learning and deep learning, see \cite{RN312,he2016deep}. 
 The work \cite{drusvyatskiy2018efficiency}
gave a complete recipe of complexity analysis of accelerated proximal-linear
methods for deterministic optimization. Momentum and accelerated methods for convex stochastic optimization can be referred from \cite{loizou2020momentum, sebbouh2020convergence} .

\textbf{Paper Outline}
The paper is organized as follows.  Section~\ref{sec:background} introduces necessary backgrounds and basics of stochastic model-based optimization. 
Section~\ref{sec:minibatch} presents the minibatch stochastic
model-based methods. Based on a novel error analysis of stochastic
model approximation, Section~\ref{sec:minibatch} establishes a
sublinear rate of convergence to certain optimality measure. Section~\ref{sec:momentum}
presents a new stochastic model-based method with an extrapolation
step to involve Polyak-type momentum; a new Lyapunov analysis is developed to show convergence complexity under a specific optimality measure.
Section~\ref{sec:Experi} conducts experimental study to illustrate the empirical advantage
of our proposed methods. Finally, Section~\ref{sec:Conclu} draws
conclusions. Missing proofs are available in  Appendix sections.

